Advanced-Step Real-time Iterations with Four Levels -- New Error Bounds and Fast Implementation in acados

The Real-Time Iteration (RTI) is an online nonlinear model predictive control algorithm that performs a single Sequential Quadratic Programming (SQP) per sampling time. The algorithm is split into a preparation and a feedback phase, where the latter one performs as little computations as possible solving a single prepared quadratic program. To further improve the accuracy of this method, the Advanced-Step RTI (AS-RTI) performs additional Multi-Level Iterations (MLI) in the preparation phase, such as inexact or zero-order SQP iterations on a problem with a predicted state estimate. This paper extends and streamlines the existing local convergence analysis of AS-RTI, such as analyzing MLI of level A and B for the first time, and significantly simplifying the proofs for levels C and D. Moreover, this paper provides an efficient open-source implementation in acados, making it widely accessible to practitioners.

==> table_clc_benchmark.tex <==
\begin{table}
\centering
\caption{Timings, relative suboptimality, stationarity residual and constraint violation for different controllers. \label{tab:asrti_experiment}}
\vspace{-.2cm}{\footnotesize
\begin{tabular}{lrrrrrr}
\toprule
& \multicolumn{2}{c}{max. timings [ms]} & rel. sub- & \multicolumn{2}{c}{mean}\\
algorithm & preparation & feedback &  opt. [\%] & $10^3 \norm{g} $ & $\nabla_w\mathcal{L}$ \\ \midrule
SQP-100&\textbf{0.00} &5.518 &\textbf{0.05} &0.00 &0.00\\
SQP-2&\textbf{0.00} &0.264 &\textbf{0.25} &12.99 &7.75\\
AS-RTI-D-2&0.35 &\textbf{0.020} &\textbf{0.04} &0.74 &1.28\\
AS-RTI-D-1&0.23 &\textbf{0.020} &\textbf{0.25} &8.26 &5.38\\
AS-RTI-C-2&0.32 &\textbf{0.020} &\textbf{0.04} &5.34 &2.20\\
AS-RTI-C-1&0.23 &\textbf{0.021} &\textbf{0.24} &10.70 &5.85\\
AS-RTI-B-2&0.28 &\textbf{0.021} &\textbf{0.57} &1.28 &8.20\\
AS-RTI-B-1&0.19 &\textbf{0.021} &\textbf{0.54} &8.77 &7.98\\
AS-RTI-A&0.13 &\textbf{0.019} &\textbf{0.54} &12.41 &6.63\\
RTI&0.11 &\textbf{0.022} &3.55 &14.06 &8.26\\
\bottomrule
\end{tabular}
\vspace{-.4cm}}
\end{table}

